Mixing Consistent Deep Clustering

Finding well-defined clusters in data represents a fundamental challenge for many data-driven applications, and largely depends on good data representation. Drawing on literature regarding representation learning, studies suggest that one key characteristic of good latent representations is the ability to produce semantically mixed outputs when decoding linear interpolations of two latent representations. We propose the Mixing Consistent Deep Clustering method which encourages interpolations to appear realistic while adding the constraint that interpolations of two data points must look like one of the two inputs. By applying this training method to various clustering (non-)specific autoencoder models we found that using the proposed training method systematically changed the structure of learned representations of a model and it improved clustering performance for the tested ACAI, IDEC, and VAE models on the MNIST, SVHN, and CIFAR-10 datasets. These outcomes have practical implications for numerous real-world clustering tasks, as it shows that the proposed method can be added to existing autoencoders to further improve clustering performance.

==> __old__sections/1_abstract.tex <==
\begin{abstract}
Finding well-defined clusters in data represents a fundamental challenge for many data-driven applications, and largely depends on good data representation. Drawing on literature regarding representation learning, studies suggest that one key characteristic of good latent representations is the ability to produce semantically mixed outputs when decoding linear interpolations of two latent representations. We propose the Mixing Consistent Deep Clustering \acronym method which encourages interpolations to appear realistic while adding the constraint that interpolations of two data points must look like one of the two inputs. By applying this training method to various clustering (non-)specific autoencoder models we found that havgin the proposed training method systematically changed the structure of learned representations of a model and it improved clustering performance for the tested ACAI, IDEC, and VAE models on the MNIST, SVHN, and CIFAR-10 datasets. These outcomes have practical implications for numerous real-world clustering tasks, as it shows that the proposed method can be added to many different autoencoders to further improve clustering performance.
\end{abstract}



==> __old__sections/2_introduction.tex <==
%--------------------------------------
%	SECTION: Inroduction
%--------------------------------------
\section{Introduction}\label{sec:introduction}
Clustering is the process of assigning data points to groups based on similarity. It constitutes a fundamental part of many data-driven applications and over the past decades a large variety of clustering techniques have been studied \cite{rokach2005clustering, arthur2007k, paparrizos2015k}. When applying these techniques to high-dimensional data, they are typically preceded by dimensionality reduction techniques such as Principal Component Analysis (PCA) \cite{wold1987principal} and spectral methods \cite{ng2002spectral} to overcome the often prevalent limitation of data sparsity. Through recent advances in Deep Learning \cite{lecun2015deep, schmidhuber2015deep}, deep neural networks have since also been used as dimensionality reduction techniques. Among existing approaches, autoencoders \cite{hinton2006reducing} have widely been used to achieve this task by learning latent representations in an unsupervised setting. In the context of clustering, the successfully trained encoder can then be used to transform the input data into a lower-dimensional latent representation, which in turn serves as the input for clustering techniques. This combination of Deep Learning and clustering is called \textit{Deep Clustering}. Nowadays, several novel architectures emerged from this new research field, mostly by combining an autoencoder and a clustering algorithm through simultaneous optimization \cite{guo2017improved,jiang2016variational, min2018survey}.

While the end-to-end optimization shows promising results, a limitation of this approach is that the models are solely trained towards creating non-ambiguous clusters. In other words, they maximize the distance between already existing clusters by minimizing a data point’s distance to its assigned cluster centroid. However, they do not change the learned position of latent representations in a way that it would create more \textit{disentangled} clusters. Disentanglement refers to how well the underlying factors of variation are separated \cite{bengio2013representation}. One relevant characteristic of disentanglement in the context of clustering is the occurrence of natural clusters. It is suggested that natural clusters may occur because the local variations on a manifold tend to reflect a single category, and a linear interpolation between datapoints of different classes involves going through a low density region \cite{bengio2013representation} (see Figure \ref{fig:interpolation} for a schematic illustration). Thus, while traversing the linearly interpolated path between instances of two clusters, one should not encounter instances of a third cluster. Since the positions of the lower-dimensional feature representations are learned, this interpolation characteristic can be learned as well. This training method, often referred to as \textit{interpolation training}, has been used in supervised settings to increase the robustness of a classifier \cite{verma2018manifold,guo2019mixup} as well as in a semi-supervised setting to achieve comparable performance with fewer class instances \cite{verma2019interpolation, berthelot2019mixmatch}. 

This paper proposes makes use of this interpolation training technique in an unsupervised setting. To ensure that the output of the decoder given the mixed representation resembles the data distribution at a pixel level, we leverage adversarial learning (Goodfellow et al., 2014), where here we train a discriminator to distinguish between decoded mixed and real data points. Additionally, we explicitly enforce the desideratum of linear dependencies between clusters in the latent space by adding an additional constraint to the overall loss function of the autoencoder, which realizes a structure that is better suited for downstream clustering tasks. This new framework, called \acronym, can be applied to preexisting convolution-based autoencoder models to further improve clustering performance. In summary, the contributions of this work are as follows:
\begin{itemize}
    \item We combine the approaches of interpolation training and adversarial learning with the explicit enforcement of a desired structure in the latent space.
    \item Experimentally, we show that \acronym outperforms all other tested models with regard to clustering results on the MNIST, SVHN and CIFAR-10 datasets (section \ref{sec:results}).
    \item We empirically show that this improved framework can be added to various autoencoder architectures to improve clustering performance.
\end{itemize}



\begin{comment}
In an unsupervised setting, a recent method called Adversarially Constrained Autoencoder Interpolation (ACAI) has been proposed \cite{berthelot2018understanding} which uses interpolations of latent representations combined with an adversarial regularizer to train an autoencoder. Without any clustering-specific loss, this training procedure managed to create a latent space structure that is on-par with current state-of-the-art deep clustering models with regard to clustering accuracy. However, although the authors expect that the interpolated points will move from the first datapoint to the second datapoint in a semantically meaningful way, they do not explicitly enforce this expectation in the loss function of the autoencoder. To make the desideratum of linear dependencies between clusters more explicit, an additional constraint can be added to the overall loss function of the autoencoder.

The current paper combines both a recently introduced training regime and an additional constraint in the loss function to create an autoencoder based framework that improves clustering performance. Drawing on recent studies on \textit{interpolation training} \citep{verma2018manifold, verma2019interpolation}, we build on top of the ACAI framework \citep{berthelot2018understanding} by adding a constraint to the loss term that is expected to enforce a more cluster-friendly structure onto the feature space. 

This new framework, called \acronym, can be applied to preexisting convolution-based autoencoder models to further improve clustering performance. In summary, the contributions of this work are as follows:
\begin{itemize}
    \item We combine both approaches of enforcing structure on a feature space by including adversarially constrained interpolation training and an additional constraint in the loss term
    \item Experimentally, we show that \acronym outperforms all other tested models including the ACAI framework with regard to clustering results on the MNIST, SVHN and CIFAR-10 datasets (section \ref{sec:results});
    \item We empirically show that this improved framework can be added to various autoencoder architectures to improve clustering performance.
\end{itemize}
The remaining paper is structured as follows: Section \ref{sec:related_work} selectively reviews relevant literature on Deep Clustering, interpolation training, and we describe the ACAI framework \cite{berthelot2018understanding}. In Section \ref{sec:methods}, we describe the limitation of ACAI with regard to clustering and we propose \acronym, a new framework that improves on this limitation. The experimental setup including datasets and evaluation metrics are explained in Section \ref{sec:experiments}. Section \ref{sec:results} reports the results from the conducted experiments. We interpret and discuss the results in Section \ref{sec:discussion} and, last but not least, we draw conclusions in Section \ref{sec:conclusion}. 
\end{comment}

==> __old__sections/3_related_work.tex <==
%--------------------------------------
%	SECTION: RELATED WORK
%--------------------------------------
\section{Related Work}\label{sec:related_work}

\subsection{Deep Clustering}
Recent work in Deep Clustering started to focus on creating a clustering-friendly feature space through the simultaneous minimization of reconstruction and clustering loss. As one of the first to combine both steps into an end-to-end framework, Xie and colleagues \citep{guo2017improved} published the \textit{Improved Deep Embedded Clustering} (IDEC) model, a method that simultaneously learns feature representations and cluster assignments using an autoencoder. It first pretrains the autoencoder by using a reconstruction loss and then fine-tunes the network by adding a cluster assignment hardening loss, where each point is assigned a probability of belonging to a given cluster. This simultaneous optimization approach significantly increased clustering accuracy compared to separate autoencoder and clustering optimization \citep{guo2017improved}. Nowadays, the architecture of the IDEC model is typically used as a basis for clustering-specific autoencoder models and it has been extended to generative models such as variational autoencoders (VAE) \cite{kingma2013auto} and generative adversarial networks (GAN) \cite{goodfellow2014generative}. For example, \cite{jiang2016variational} developed the \textit{variational deep embedding} (VaDE) framework, which simultaneously optimizes a Variational Autoencoder and a clustering-specific Gaussian Mixture Model (GMM). This results in a significant improvement in clustering accuracy as they were able to outperform the standard GMM clustering method, VAE and GMM networks with separate optimization as well as other deep clustering methods \cite{jiang2016variational}.

\subsection{Interpolation Training}\label{sec:interpolation_training}
Learning good representations is an active field of research in itself \cite{bengio2013representation} and primarily investigates how to learn representations that are \textit{disentangled}. Since a disentangled representation unravels the underlying structure, it displays several attributes that are useful in the context of clustering, most importantly lower dimensional manifolds, naturally occurring clusters, and a simplicity of factor dependencies (for a comprehensive list of attributes, see \cite{bengio2013representation}). One common denominator across these attributes is the ability to linearly interpolate between clusters or data points of classes while traversing low density regions. Since the representations of data points in the latent space are learned, it is possible to enforce this interpolation characteristic through training. For example, recent work \cite{verma2018manifold} applied an interpolation training method called Manifold Mixup in a supervised setting to learn robust features. By interpolating two data points' hidden layer activations, the learned class-representations were more discriminative, compact, and had fewer directions of variance, suggesting that the model learned more disentangled representations.


\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.60]{Figures/adv_horizontal_3.png}
    \caption{An illustration of a clustering specific autoencoder combined with the \acronym training method. The latent vectors of two input datapoints are used for three purposes, (1) they are sent to the clustering-specific loss, (2) they are used for interpolation (see Section \ref{sec:methods_acai}), (3) they are sent to the decoder to create reconstructions of the input.}
    \label{fig:acai+}
\end{figure*}

==> __old__sections/4_method.tex <==

%--------------------------------------
%	SECTION: ACAI and ACAI+
%--------------------------------------
\begin{comment}

\section{Method}\label{sec:methods}
\subsection{ACAI}\label{sec:methods_acai}
Recently, Berthelot and colleagues \citep{berthelot2018understanding} proposed a method to apply interpolation training in an unsupervised setting. In their ACAI framework, interpolating describes the process of using an encoder $f_{\phi} (x)$ to map datapoints onto a lower-dimensional latent representation $z$. A decoder $g_{\theta}(z)$ is then used to reconstruct a mixture of two latent representations. For two datapoints $x_1$ and $x_2$, the linear interpolation $z_{\alpha}$ is calculated as:
\begin{equation}
    z_{\alpha} = \alpha \cdot f_{\phi} (x_1) + (1 - \alpha) \cdot f_{\phi} (x_2)
\end{equation}
for some $\alpha \in [0,1]$. The resulting interpolated representation $z_{\alpha}$ is then reconstructed by the decoder $\hat{x}_{\alpha} = g_{\theta} (z_{\alpha})$. Ideally, adjusting $\alpha$ from 0 to 1 will produce a sequence of realistic datapoints where each subsequent $\hat{x}_\alpha$ is progressively less semantically similar to $x_1$ and more semantically similar to $x_2$. Then, a second encoder network $d_{\omega}$, called a \textit{critic} or \textit{adversarial regularizer}, is fed these interpolants and its goal is to predict the mixing coefficient $\alpha$ that was used to generate the decoded signal. More formally, it outputs a scalar value and is trained to minimize
\begin{equation}\label{eq:lossDiscriminator}
    L_d = ||d_\omega (\hat{x}_\alpha) - \alpha ||^2 + ||d_\omega (\gamma x + (1 - \gamma)\hat{x}||^2
\end{equation}
where $\gamma$ is a scalar hyperparameter. The first part of the equation calculates the MSE between the predicted and true $\alpha$ values whereas the second part of the equation predicts the $\gamma$ hyperparameter that is used to interpolate between the input image $x$ and the reconstruction $\hat{x}$ \footnote{\cite{berthelot2018understanding} suggest that this second term may not be necessary but helps to stabilize the training process in the early training phase.}. Simultaneously, the autoencoder is trained to fool the critic to think that the $\alpha$ value is always zero and it receives the critic's performance as feedback in terms of a loss. Consequently, the overall loss of the autoencoder is
\begin{equation}\label{overallAutoencoderLoss}
    L_{f,g} = || x - g_{\theta}(f_{\phi}(x)) ||^2 + \lambda ||d_\omega (\hat{x}_\alpha) ||^2
\end{equation}
where $\lambda$ is a hyperparameter that determines how strongly the critic's performance contributes to the overall autoencoder loss. Empirically, this approach resulted in realistic and smooth interpolations of the autoencoder's latent space as well as in increased clustering accuracy \cite{berthelot2018understanding}.


%% Novel Contribution / Limitation
To illustrate the limitation of the ACAI framework in the context of clustering, we first discuss an example of linear interpolations between four classes, depicted in figure \ref{fig:interpolation}. 

When interpolating between two clusters, for example from cluster B to cluster C, the resulting interpolant will likely look like a realistic data point of cluster B and become less semantically similar to B and more semantically similar to C as a function of increasing $\alpha$. Since an interpolant always has to look like a realistic datapoint, interpolants close to cluster B will look like a real data point from B whereas an interpolant close to cluster C will look like a real datapoint from C, visualized as blurred versions of the cluster's datapoints in figure \ref{fig:interpolation}. However, let's consider the outlier of cluster B at the right end of the coordinate system. If we'd like to interpolate this data point with another data point from cluster C, the interpolants with an $\alpha \approx 0.5$ will not necessarily look like a real data point from the clusters B or C, but instead it would look like a data point coming from cluster D. This is because, for $\alpha \approx 0.5$, the position of the interpolated data point would lie in the area where most data points belong to cluster D (bottom right quadrant of the coordinate system in figure \ref{fig:interpolation}) and, therefore, through interpolations of data points from D with other clusters, interpolants in this quadrant will look most similar to D. Since the interpolant will look like a realistic datapoint, the critic will output $\alpha = 0$ and the overall loss of the autoencoder in the ACAI framework will not increase. In other words, any realistic looking interpolant between cluster C and B will correspond to an inability of the critic to guess the used $\alpha$ value. 

However, this behaviour would not explicitly enforce linear dependencies between clusters, which is an important characteristic of disentangled representations \cite{bengio2013representation}. Additionally, this also means that the network would not necessarily need to create more disentangled clusters because the described behaviour would not enforce the creation of low density regions between clusters. In the above scenario, the outlier from cluster B does not have any 'incentive' to move towards the cluster centroid but can stay at its position. Instead, we would like the data point to move towards the centroid position to enforce lower density regions between clusters.

% \begin{figure}[h]
% \centering
% \includegraphics[width=6cm,height=5cm]{Figures/interpolation_WITHOUT_GRAD.png}
% \caption[Example Interpolation]{Illustration of linear interpolations and low-density regions between four clusters of classes.} 
% %To satisfy the condition of low-density regions between clusters, interpolations must look like coming from the cluster of the first datapoint for $\alpha \geq 0.5$ and while looking like coming from the cluster of the second datapoint for $\alpha \leq 0.5$.
% \label{fig:interpolation}
% \end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=6cm,height=5cm]{Figures/interpolation_WITHOUT_GRAD.png}
\caption[Example Interpolation]{Illustration of linear interpolations and low-density regions between four clusters of classes.} 
%To satisfy the condition of low-density regions between clusters, interpolations must look like coming from the cluster of the first datapoint for $\alpha \geq 0.5$ and while looking like coming from the cluster of the second datapoint for $\alpha \leq 0.5$.
\label{fig:interpolation}
\end{figure}

\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.4]{Figures/acai_vs_acai+/two_MNIST_all.png}
    \caption[Example Interpolation]{The models' learned data point positions in the two-class MNIST example.}
    \label{fig:two_mnist_example}
\end{figure*}


\subsection{\name (\acronym)}
To enforce the desideratum of linear dependencies between clusters and thereby overcome the described limitation of ACAI, we propose an improved version, called \textit{\name} (\acronym). \acronym introduces an additional constrained that is added to the overall loss function of the autoencoder. More specifically, when linearly interpolating between $x_1$ and $x_2$, the interpolants for $\alpha \in [0, 0.5]$ must look like $x_1$ whereas the interpolants for $\alpha \in [0.5, 1]$ must look like $x_2$. Formally, this can be expressed by:
\begin{equation}
    z_\alpha = (1 - \alpha) f_\phi (x_i) + \alpha f_\phi (x_j)
\end{equation}
\begin{equation} \label{eq:addedConstraint}
    L = || x_i - g_{\theta}(z_{\alpha}) ||^2   
\end{equation}
where $\alpha \in [0, 0.5]$. Consequently, we define the overall loss function of the autoencoder as follows:
\begin{equation}
    L_{i} = || x_i - g_{\theta}(f_{\phi}(x_i)) ||^2 + \lambda ||d_\omega (\hat{x}_\alpha) ||^2 + || x_i - g_{\theta}(z_{\alpha}) ||^2
\end{equation}
This overall loss should enforce that all clusters can linearly interpolate between each other and, in addition, that all interpolants look like coming from the respective data points that were used for the interpolation. Turning to the interpolation between the outlier of cluster B and a data point from C, the resulting interpolant will look like a realistic data point from D, which is not one of the input images and, as a consequence, the autoencoder loss will increase. Since every position in the coordinate system can only store a single representation (i.e. the position of the interpolant in the coordinate system can only be decoded deterministically as a datapoint coming from one of the clusters B, C, or D), there will be a conflict of assigning different representations to the same position. As the datapoint locations are learned through training, it is expected that the pressure to decode consistent representations at interpolated positions causes the outlier from cluster B to move towards the centroid position of cluster B. Eventually, this would lead to more disentangled clusters and lower-density regions between the clusters.


\subsection{ACAI vs. \acronym} \label{sec:acaiVSacai+}
To provide additional intuition on how the added constraint changes the learned positions of the data points in the latent space, we illustrate the difference in behaviour using a toy dataset. More specifically, we made use of a smaller version of the MNIST dataset and sub-selected two classes from that dataset. we trained three autoencoders (a baseline version, the original ACAI method and the proposed \acronym method) with a latent dimensionality of 2 in order to visualize the learned positions of the data points without manipulating the values with a dimensionality reduction technique. For better comparison between models, the axes were kept at the same scale across figures.

In the left panel of figure \ref{fig:two_mnist_example} it shows the plotted positions of the data points for the baseline version. As can be seen in the figure, the individual data points are rather scattered across the space since there is no loss enforcing a more compact representation. In contrast to that, the center panel shows the learned positions of the ACAI model, which enforces the data points to be positioned more compactly. Furthermore, since interpolants do not have to look like the input images but only like a realistic data point, the autoencoder makes use of this by arranging the lines in a more "linear" fashion. This, in turn, leads to more "semantically meaningful" interpolations as described in \cite{berthelot2018understanding}.

Generally, this distribution of learned positions seems favourable. Since fewer principal components are needed to explain a class's variance, it suggests a more disentangled representation of the data points. However, for traditional clustering algorithms such as k-Means, this distribution of data points is not preferable since the ratio of in-class to between-class distances is sub-optimal. Thus, in order to improve clustering, it would be beneficial if all points of a given class would lie close to each other.

As shown in the right panel of figure \ref{fig:two_mnist_example}, the \acronym method learned more compact positions of the data points. The ratio between in-class distances and between-class distances significantly changes which, in turn, improves subsequent clustering performance. Additionally, it is worth noting that the overall distribution of the data point positions changes as well as the amount of principal components that are necessary to describe the clusters. When using the original ACAI approach, most of the variance can be explained by a single component that's almost parallel to the x-axis. When using the \acronym approach, however, two components are needed in order to explain the data's variance accurately, as seen for class 0 in the figure.
\end{comment}

==> __old__sections/5_experiments.tex <==
\section{Experiments} \label{sec:experiments}
In this section, we demonstrate the effectiveness and validation of the proposed method on three benchmark datasets. We provide quantitative comparisons of \acronym with other Autoencoder models. More specifically, we compare it against the ACAI framework to investigate if the added loss term improves clustering performance, a convolutional VAE model to see if the \acronym framework can be combined with generative models, and the IDEC model to find out if the\acronym framework can further improve on clustering-specific autoencoder models. The last two were trained twice, with and without the \acronym framework, and all models are based on the same encoder and decoder architecture. The code of \acronym is available at https://github.com/kdd20-submission/\acronym.


%-----------------------------------
%	SECTION: Datasets
%-----------------------------------
\subsection{Datasets} \label{sec:method_datasets}
The following datasets were used in the experiments:

\begin{itemize}
    \item \textbf{MNIST}: The "Modified National Institute of Standards and Technology" (MNIST) dataset was first published in 1998 \cite{lecun1998mnist} and is one of the most widely used benchmark datasets. It consists of 70,000 greyscale, handwritten digits representing 10 classes, separated into 60,000 training images and 10,000 test images. The images are centered and of size 28 by 28 pixels. In order to keep the same input dimensions for all datasets, the MNIST images are resized to 32 x 32 pixels using bilinear interpolation.
    
    \item \textbf{SVHN}: The "Street View House Numbers" (SVHN) dataset consists of around 73,257 and 26,032 colored training and test images, respectively. The images depict house numbers cropped from Google Street View. They represent 10 different classes and are of size 32 by 32 pixels (\cite{netzer2011reading}).
    
    \item \textbf{CIFAR10}: The "Canadian Institute For Advanced Research" (CIFAR) developed two datasets of different sizes. For the present thesis, the CIFAR-10 dataset will be used, which consists of 60,000 colored images of 32 x 32 pixels and 10 classes representing various objects including frogs, planes, and cars \cite{krizhevsky2009learning}.
\end{itemize}

\subsection{Experimental Setup}\label{sec:method_models}
\subsubsection{General Autoencoder Architecture}
For an overview of the general autoencoder architecture, see Figure \ref{fig:overall_arch} in Appendix A.

The overall structure includes blocks of two consecutive 3 x 3 convolutional layers where the number of channels is doubled between the first and second layer of a given block (see Appendix A, Figure \ref{fig:conv_blocks}). All convolutions are zero-padded to keep equal input and output shapes. Also, every block, except the last one, is followed by 2 x 2 average pooling. The final layer is used as the latent representation and therefore does not use an activation function while all previous layers use a leaky ReLU nonlinearity \cite{maas2013rectifier} with a negative slope of $a = 0.2$. For all experiments, the above-described blocks are repeated 3 times, resulting in a latent dimensionality of 256.

The decoder is created symmetrically to the encoder with respect to layer architecture, however, the average pooling function is substituted by 2 x 2 nearest neighbour upsampling \cite{odena2016deconvolution}. All parameters are initialized as zero-mean Gaussian random variables with the standard deviation:
\begin{equation}
    std = \sqrt{\frac{2}{(1 + a^2) * \text{fan\_in}}}
\end{equation}
where $a$ is the negative slope of the rectifier and fan\_in represents the number of incoming neurons from the previous layer. All models are trained with a batch size of 64 and parameters are optimized using Adam \cite{kingma2014adam} with a learning rate of 0.0001 and default values for $\beta_1$, $\beta_2$, and $\epsilon$. Across all datasets, every model is trained for a total duration of 400 epochs.

% AE architectures overview
\begin{table}
  \caption{Overview of the different autoencoder models}
  \label{table:aeOverview}
  \begin{tabular}{l c c c c}
    \toprule
    Model&AE Loss&Adv. Loss*&Constraint**&Cl. Loss\\
    \midrule
        VAE & ELBO & - & - & - \\
        IDEC & MSE & - & - & KLD on SCA \\
        ACAI & MSE & yes & -  & - \\
        \acronym & MSE & yes & yes & - \\
        \acronym+IDEC & MSE & yes & yes & KLD on SCA \\
        \acronym+VAE & ELBO & yes & yes & - \\
  \bottomrule
\multicolumn{5}{l}{\textit{Notes.} KLD = KL-divergence, SCA = Soft Cluster Assignment}\\
\multicolumn{4}{l}{* eq. \ref{eq:lossDiscriminator}, ** eq. \ref{eq:addedConstraint}}\\
\end{tabular}
\end{table}

% AE architectures overview
\begin{table}
  \caption{Overview of the different autoencoder models}
  \label{table:aeOverview}
  \begin{tabular}{l c c c c}
    \toprule
    Model&AE Loss&Adv. Loss*&Constraint**&Cl. Loss\\
    \midrule
        ACAI & MSE & yes & -  & - \\
        ACAI+ & MSE & yes & yes & - \\
        IDEC & MSE & - & - & KLD on SCA \\
        IDEC+ & MSE & yes & yes & KLD on SCA \\
        VAE & ELBO & - & - & - \\
        VAE+ & ELBO & yes & yes & - \\
  \bottomrule
\multicolumn{5}{l}{\textit{Notes.} KLD = KL-divergence, SCA = Soft Cluster Assignment}\\
\multicolumn{4}{l}{* eq. \ref{eq:lossDiscriminator}, ** eq. \ref{eq:addedConstraint}}\\
\end{tabular}
\end{table}


\subsubsection{Baseline Autoencoder (AE)}
The first model is the baseline model. It is the simplest of the studied autoencoders and is used as a baseline that other models are compared against. The encoder as well as the decoder use the layer architecture and training procedure described above. In our experiments, the network tries to minimize the mean-squared error loss between the input $x$ and reconstruction $\hat{x}$.

\subsubsection{Improved Deep Embedded Clustering (IDEC)}
The IDEC architecture \cite{guo2017improved} is almost identical to the baseline autoencoder and it uses the same training procedure as the baseline autoencoder during pre-training. During the fine-tuning phase, however, an additional clustering loss is added to the overall loss of the autoencoder. This clustering loss, called "cluster assignment hardening loss", consists of the KL-divergence loss of the soft cluster assignments \cite{guo2017improved}.

\subsubsection{Variational Autoencoder (VAE)}
The third model that is used is the variational autoencoder \cite{kingma2013auto}. The VAE differs from the baseline autoencoder by introducing a constraint over the latent representation $z$, thereby imposing a probabilistic prior distribution $p(z)$. This way, the encoder $f_\phi(x)$ learns to approximate the posterior distribution $p(z|x)$ and the decoder $g_\theta(z)$ learns to reconstruct $x$ by parametrizing the likelihood $p(x|z)$. The encoding and decoding layers as well as the training procedure remain the same as for the previous models. However, the loss function differs as it tries to maximize the likelihood of a given sample $x$ while enforcing a latent distribution through a KL-divergence loss. To make the training procedure practically feasible, $p(z|x)$ is commonly modelled as a diagnoal covariance Gaussian, which makes it possible to use the "reparametrization trick", which replaces $z \sim \mathcal{N}(\mu,\,\sigma I)$ with $\epsilon \sim \mathcal{N}(0,\, I)$ and $ z = \mu + \sigma * \epsilon$ where $\mu, \sigma \in \mathbf{R}^{d_z}$ are the predicted mean and standard deviation produced by $f_\phi$.

\begin{figure*}[hbt!]
\centering
    {\includegraphics[scale=0.5]{Figures/acai_vs_acai+/baseline_PCA_AVERAGES_epoch_400.png}}
    \qquad
    {\includegraphics[scale=0.5]{Figures/acai_vs_acai+/base_mine_PCA_AVERAGES_epoch_400.png}}
\caption[PCA across classes]{PCA across classes. The left panel (a) shows the PCA performance for the baseline model and the right panel (c) depicts the principal components for the \acronym model.}
\label{fig:illustration_mnist_pca}
\end{figure*}

\subsubsection{Adversarially Constrained Interpolation (ACAI)} \label{critic_section}
The ACAI model consists of two networks: the first network is the baseline autoencoder described above and the second network is a critic, which has the same architecture as the encoder part of the autoencoder. However, the last layer of the critic, which represents the latent representation $z \in \mathcal{R}^{d_z}$, is flattened and the mean value is taken as the $\alpha$ prediction.

The critic receives the reconstructed image of an interpolation and learns to predict the alpha value that was used to interpolate the two input images. In other words, the network tries to minimize the difference between its prediction and the true alpha value (equation \ref{eq:lossDiscriminator}) while the autoencoder is trained to fool the critic into always outputting $\alpha = 0$. This adds a second term to the loss of the autoencoder, leading to the overall loss shown in equation \ref{overallAutoencoderLoss}.

\subsubsection{\name (\acronym)}
Figure \ref{fig:acai+} shows the overall framework of \acronym including a clustering specific loss (e.g. combining \acronym with IDEC). The overall architecture of the \acronym model is similar to the ACAI model described above. However, a second constraint is added to the autoencoder, such that when linearly interpolating between $x_1$ and $x_2$, the interpolants for $\alpha \in [0, 0.5]$ must look like $x_1$ while the interpolants for $\alpha \in [0.5, 1]$ must look like $x_2$ (see eq. \ref{eq:addedConstraint}).

\subsubsection{\acronym+IDEC and \acronym+VAE}
To address the question if the \acronym framework can be combined with generative-, and clustering-specific autoencoder models, the IDEC and VAE were also trained with the \acronym framework, resulting in the \acronym+IDEC and \acronym+VAE models. For an illustration of the \acronym+IDEC framework, see Figure \ref{fig:acai+}.

%-----------------------------------
%	SECTION: Evaluation Metrics
%-----------------------------------
\subsection{Evaluation Metrics} \label{sec:method_evaluation}
As noted in \cite{guo2017improved, min2018survey}, clustering methods are commonly evaluated by clustering accuracy (ACC) and Normalized Mutal Information (NMI). We used the K-means algorithm with Euclidean distance as the distance metric. Since this algorithm is sensitive to each dimension’s relative variance, we normalized the variance prior to clustering by performing PCA whitening on the latent representations. The algorithm was run 1000 times with different random initializations and the run with the best objective value was used to calculate the accuracy and NMI of the resulting clusters. To calculate the clustering accuracy, a dataset's labels were used, as they were not used while training the model. The accuracy corresponds to the optimal one-to-one mapping of cluster IDs to classes as determined by the Hungarian algorithm \cite{kuhn2005hungarian}. This results in the following equation:
\begin{equation}\label{eq:acc}
    ACC = \underset{m}{max} \frac{\sum_{i=1}^n 1(y_i = m(c_i))}{n}
\end{equation}
where $c_i$ is the model's cluster assignment, $m$ is a mapping function that covers all possible one-to-one mappings between assignments and labels, and $y_i$ is the ground-truth label. 

The second metric used in the cluster evaluation is \textit{Normalized Mutual Information (NMI)} (Estevez et al., 2009), which is a way of calculating cluster purity. Given a dataset containing ground-truth labels $Y$ and cluster labels $C$, each cluster can be assigned to the majority class in that cluster. Then, the mutual information score $I(Y, C)$ can be computed, which corresponds to the amount of information that is gained about $Y$ through observing $C$. If the mutual information score is 0, receiving the cluster label of a data point does not tell us anything about its ground-truth label whereas a score of 1 would represent a perfect recreation of the classes. However, this measure does not correct for the total amount of clusters, which means that if the number of clusters $K = N$, it would yield a perfect score. Thus, the NMI calculates the mutual information and then normalizes it by the amount of entropy $H$ since entropy tends to increase with the number of clusters. This results in the overall function:

\begin{equation}\label{eq:nmi}
    NMI(Y, C) = \frac{I(Y,C)}{\frac{1}{2}[H(Y) + H(C)]}.
\end{equation}



==> __old__sections/6_results.tex <==
\section{Results}\label{sec:results}

The results section is structured as follows: we start by quantifying the intuition we presented in section \ref{sec:acaiVSacai+} of how ACAI and \acronym differ in the shape and structure they learn for the latent representations. Then, we show the latent embeddings learned by the models and how they performed on clustering the various datasets.

\begin{table}[h]
    \caption{Average clustering accuracy as measured by ACC and NMI (higher is better). Clusters were calculated using 1000 random initializations of K-means on the feature space of the given autoencoder.}
    \centering
    \begin{tabular}{l c c c}
        \toprule
        Model & MNIST & SVHN & CIFAR-10\\
        \midrule
            ACAI & 90.08 / 88.60 & 22.00 / 15.17 & 20.30 / 09.29  \\
            \acronym & 96.39 / 92.39 & \textbf{35.00} / \textbf{43.28} & \textbf{25.99} / \textbf{16.41} \\
            IDEC & 66.03 / 72.77 & 17.97 / 05.65 & 21.75 / 09.74 \\
            \acronym+IDEC & \textbf{97.61} / \textbf{93.80} & 18.36 / 09.74 & 22.17 / 10.73  \\
            VAE & 82.44 / 88.68 & 11.64 / 00.47 & 20.86 / 10.61 \\
            \acronym+VAE & 84.95 / 89.63 & 15.24 / 01.47 & 20.85 / 09.81 \\
        \bottomrule
    \end{tabular}
    \label{tab:clusteringResults}
\end{table}

%% MNIST INTERPOLATIONS
\begin{figure*}[h]
\centering
\includegraphics[scale=1.0]{Figures/results_embeddings/interps_mnist.png}
\caption[MNIST Interpolations]{Interpolations on the MNIST dataset. The panels (a) - (f) show interpolations of the various autoencoders as follows: (a) ACAI, (b) \acronym, (c) IDEC, (d) \acronym+IDEC, (e) VAE, (f) \acronym+VAE.}
\label{fig:interps_mnist}
\end{figure*}

\subsection{ACAI vs \acronym}\label{sec:ch4_acaiVSacai+}
To investigate if the earlier presented intuition can be confirmed in high-dimensional latent spaces, we quantified the shape of the learned embeddings through Principal Component Analysis. To do this, we trained a baseline autoencoder as well as ACAI and \acronym on the MNIST dataset. Then, we sub-selected all data points of a given class and encoded the images to receive latent vectors for all images of that class. Subsequently, we performed a PCA on these latent vectors with a self-selected cutoff of 40 in order to obtain the most relevant principal components. After doing this for every class, the components of all classes were normalized and averaged. 

The result of this procedure is shown in figure \ref{fig:illustration_mnist_pca}. In the left panel, the principal components of the baseline model are presented, while the same analysis for the ACAI model is shown in the center panel and the results for the \acronym model are illustrated in the right panel. The first component of the ACAI method explains a visibly larger amount of variance compared to its second component as well as compared to the first component of the baseline and \acronym methods. Additionally, the standard deviation of the principal components of the ACAI method is visibly higher compared to the other two methods, suggesting that there are significant differences in principal components' contributions between classes. The differences between the individual components for the \acronym model are in general smaller than for the ACAI model. This difference is in line with the intuition outlined in Section \ref{sec:acaiVSacai+} and we will discuss this finding and its implications about the clusters' shapes in Section \ref{sec:discussion}.


\subsection{Clustering Performance}
The clustering results are shown in table \ref{tab:clusteringResults} and the corresponding PCA embeddings for MNIST are depicted in figure \ref{fig:pca_mnist}. On the MNIST dataset, the combination of the deep clustering model IDEC combined with \acronym training led to the best clustering performance with an accuracy of 97.61\% and an NMI of 93.80\%. On the SVHN as well as CIFAR10, the \acronym model achieved the best performance in terms of accuracy and NMI. Across all datasets, the \acronym model performed better than the ACAI model, suggesting that the additional constraint (eq. \ref{eq:addedConstraint}) indeed improves clustering performance. Additionally, the models that were trained without and with \acronym (i.e. IDEC and VAE) improved in clustering performance when the \acronym training method was added. This empirical result is present across all datasets, suggesting that adding \acronym to an existing autoencoder model further improves clustering performance of a given autoencoder model.

%% PCA ON MNIST
\begin{figure}[h]
\centering
\includegraphics[scale=0.52]{Figures/results_embeddings/PCA_mnist.png}
\caption[pca mnist]{First two PCA components of the learned data point positions in the latent space by the various models on the MNIST dataset.}
\label{fig:pca_mnist}
\end{figure}

\begin{comment}
%% T-SNE ON MNIST
\begin{figure}
\centering
\includegraphics[scale=1.0]{Figures/results_embeddings/tsne_mnist.png}
\caption[tsne mnist]{T-SNE embeddings of the learned data point positions in the latent space by the various models on the MNIST dataset.}
\label{fig:tsne_mnist}
\end{figure}
\end{comment}




==> __old__sections/7_discussion.tex <==
\section{Discussion}\label{sec:discussion}
As mentioned in Section \ref{sec:ch4_acaiVSacai+}, the PCA of the ACAI model is characterized by a large contribution of the first component and a steep decline in explained variance by the principal components following the first component. This result suggests that the learned positions of the data points, and the resulting class locations, can be explained using fewer dimensions compared to the baseline and \acronym models. In other words, the learned embeddings of a given class seem to have a more elongated shape while lying to a large degree on a hyperplane. This in turn suggests a more disentangled representation of the individual classes (see Section \ref{sec:interpolation_training}). 

This interpretation is in line with the previously described intuition in section \ref{sec:acaiVSacai+} and it is further supported by the visualization of the PCA of the embeddings shown in figure \ref{fig:pca_mnist}. The top left panel of the figure shows the learned positions of the embeddings of the ACAI model projected onto the first two principal components. It becomes apparent that the learned embeddings of the classes appear more "flat" as opposed to, e.g., \acronym.

In contrast to the ACAI model, the resulting PCA of \acronym (figure \ref{fig:illustration_mnist_pca}) shows that the first principal component explains overall less variance and, in addition, the drop from the first to the remaining principal components is relatively low. Instead, the explained variance is much more evenly distributed across the principal components. This suggests that the learned data points of each class need more dimensions to be explained well, which can be interpreted as a more spherical shape. This interpretation is supported by the resulting visualization in \ref{fig:pca_mnist} and it is in line with the previously illustrated example on the toy dataset in Section \ref{sec:acaiVSacai+}.

Last but not least, the PCA also shows large differences in the amount of standard deviation across classes. It appears that the ACAI model exhibits much more variation in the amount of contribution of the individual components towards the overall variance, suggesting that the exact shape of the clusters varies across classes. In contrast, the depicted standard deviations of both the baseline as well as the \acronym model are relatively small, suggesting that the resulting shape is robust across classes.

These interpretations are further supported by the accompanying interpolation and clustering results. The interpolations in figure \ref{fig:interps_mnist} illustrate that \acronym based models, especially \acronym and \acronym+IDEC, learn to decode interpolants to look like the first input image for $\alpha \geq 0.5$ while they look like the second input image for $\alpha < 0.5$. This result confirms the previously described behaviour as a consequence of adding the additional loss term. 

Furthermore, the clustering results suggest that the more spherical shape learned by \acronym may make it easier for the k-Means algorithm to correctly group the data points compared to the more elongated shape learned by ACAI. Overall, the results suggest that the added constraint of the \acronym model may facilitate more disentangled clusters compared to a baseline and ACAI model. As mentioned in section \ref{sec:interpolation_training}, a more disentangled cluster means less overlap between the individual clusters that represent semantically meaningful characteristics of the input data. Thus, adding the additional constraint seems to help create a more cluster-friendly representation.

While \acronym improved clustering performance across different models and datasets in our experiments, some questions remain unanswered. For example, we used datasets containing several balanced classes, such that we could uniformly draw samples for interpolations. Future research is needed to investigate whether whether the results obtained in the experiments generalize to datasets with class imbalances or very few classes (e.g. two classes). In these two scenario’s, randomly sampling data points for interpolations may lead to substantially more interpolations of the majority classes or, in the case of very few classes, within-class interpolations. Furthermore, recent work in the emerging field of geometric deep learning suggests that the manifold that the latent representations lie on may be curved \cite{arvanitidis2017latent} and, therefore, Euclidean distance may not be the most appropriate distance measure. Instead, it was proposed to calculate the curvature of the manifold and use the geodesic distance as a distance metric. Doing this, deep clustering performance have been reported to drastically increase \cite{shukla2019geometry,yang2018geodesic}. Since the aim of the paper was to introduce \acronym and compare it with the ACAI framework, we adopted the same evaluation metrics as \cite{berthelot2018understanding} and combining \acronym with geodesic distance measures was therefore beyond the scope. Hence, a potential line of research for future work would be to investigate how the \acronym method performs when evaluating the clustering performance using geodesic distance. 


==> __old__sections/8_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In the present paper, we improved on the original ACAI model and applied the new method, called \acronym, to various clustering (non-) specific autoencoder models. We investigated how interpolation- and adversarial training influences the learned positions of latent representations in a model's latent space and, eventually, clustering performance. We measured the models’ clustering abilities and found that adding \acronym to a model systematically changed the structure of learned representations of a model, leading to systematic increases in clustering accuracy.

Since the improvement in clustering seems to be robust across autoencoder models, existing autoencoder models can further improve in performance by adding this training method to their training pipeline. In practice, this could lead to better customer segmentation, resulting in individual recommendations based on a person's shopping behaviour. It could also improve the detection of credit card fraud since an anomaly could appear more strongly as an outlier among the normal groups of customer’s behaviour. All in all, adding the \acronym training method to existing deep clustering models could yield a great benefit for people’s lives and businesses.

==> __old__sections/A_reproducability.tex <==
\section{APPENDIX ON REPRODUCABILITY}
\subsection{Code availability}
We made our code and used Docker image publicly available on https://github.com/kdd20-submission/ACAI\_plus. 

\subsection{Experimental setup and implementation}
All experiments in this paper were performed in Python 3.7. All models were created and run using PyTorch 1.1.0, CUDA 10.0, and cuDNN 7.5. 


\subsubsection{Cluster Accuracy} We used the implementation of the Hungarian algorithm from the munkres Python package \footnote{http://software.clapper.org/munkres/}. The accuracy was then calculated using the implementation from the scikit-learn \footnote{https://scikit-learn.org/stable/modules/generated/sklearn.cluster.KMeans.html} Python package where we used 51 as random state, 1000 as maximum iteration, 1000 initializations and 6 jobs.

\subsubsection{NMI scores} The NMI scores were calculated using the implementation from the scikit-learn \footnote{https://scikit-learn.org/stable/modules/generated/sklearn.metrics.normalized\_mutual\_info\_score.html} Python package with default settings.

All models were trained and evaluated on a computing server running Ubuntu 16.04 with 64GB RAM, a GPU of type Nvidia GeForce GTX 1080 Ti with 11 GB GDDR5X RAM, and a CPU of type Intel Xeon CPU e5-2620 v2 @ 2.10ghz, providing a maximum of 12 cores. The runtime for every model per dataset is shown in Table \ref{tab:runtimes}.

%% Convolutional Blocks
\begin{figure}[h!]
\centering
\includegraphics[scale=0.8]{Figures/conv_blocks.png}
\caption[]{Convolutional blocks of the Encoder (a) and Decoder (b), respectively.}
\label{fig:conv_blocks}
\end{figure}

\begin{table}[b!]
    \caption{Runtimes for every model in hours.}
    \centering
    \begin{tabular}{l c c c}
        \toprule
        Model & MNIST & SVHN & CIFAR-10\\
        \midrule
            ACAI & 10 & 51.7 & 34.4 \\
            ACAI+ & 9.5 & 51.1 & 34.4 \\
            IDEC & 4.4 & 15.5 & 11.1 \\
            IDEC+ & 10.0 & 50.0 & 34.4 \\
            VAE & 3.9 & 17.2 & 11.7 \\
            VAE+ & 10.6 & 50.0 & 34.4 \\
        \bottomrule
    \end{tabular}
    \label{tab:runtimes}
\end{table}

%% MNIST INTERPOLATIONS
\begin{figure*}
\centering
\includegraphics[scale=1.3]{Figures/general_architeture.png}
\caption[]{Overview of the overall autoencoder architecture used across models.}
\label{fig:overall_arch}
\end{figure*}



==> __old__sections/x_formulation.tex <==

%--------------------------------------
%	SECTION: ACAI and ACAI+
%--------------------------------------
\section{\name (\acronym)}\label{sec:methods}
Let us consider an auto-encoder model $F(\cdot)$, with the encoder part denoted as $f_{\phi}(x)$ and the decoder $g_{\theta}(z)$. In an auto-encoder we wish to minimize the reconstruction, which is simply:
\begin{equation}\label{overallAutoencoderLoss}
    L_{f,g} = || x - g_{\theta}(f_{\phi}(x)) ||^2 
\end{equation}

Given an arbitrary pair of inputs, $x_i, x_j$, we would like to encode them into a lower dimensional latent representation $z_i = f_{\phi}(x_i)$ and $z_j = f_{\phi}(x_j)$, perform some combination between them through a convex combination using a mixing coefficient $z_{\alpha} = \alpha \cdot f_{\phi} (x_i) + (1 - \alpha) \cdot f_{\phi} (x_j)$ for some $\alpha \in [0,1]$, run the result through the decoder $g_{\theta}(z_{\alpha})$, and then minimise some loss function which encourages the resulting decoded mix to look realistic.

Ideally, for a pair of two inputs $\{x_1, x_2\} \in X$, $\hat{x}_{\alpha} = x_1$ for $\alpha \in [0, 0.5]$ and $\hat{x}_{\alpha}= x_2$ for $\alpha \in [0.5, 1]$.


% Let $X = \{x_1, ..., x_N\}$ with $x_n \in \mathbb{R}^D$ be the observable data that we wish to model. Further, we consider a latent variable model with latent (unobserved) variables $z \in \mathbb{R}^M, \mathbb{p}_{\theta} = $


Ideally, adjusting $\alpha$ from 0 to 1 will produce a sequence of realistic datapoints where each subsequent $\hat{x}_\alpha$ is progressively less semantically similar to $x_i$ and more semantically similar to $x_j$. With this in mind, we propose \textit{\name} (\acronym), where part of the autoencoder's objective is to produce a structure in the latent space that enforces that all clusters can linearly interpolate between each other and, in addition, that all interpolants look like coming from the respective data points that were used for the interpolation, which would lead to more disentangled clusters and lower-density regions between the clusters. The overall loss of the autoencoder can be defined as:
\begin{equation}
    L_{i} = \underbrace{|| x_i - g_{\theta}(f_{\phi}(x_i)) ||^2}_\text{reconstruction}  + \underbrace{|| x_i - g_{\theta}(\alpha f_{\phi} (x_i) + (1 - \alpha) f_{\phi} (x_j)) ||^2}_\text{enforce linearity}.
\end{equation}
Since autoencoders trained by pixel-space reconstruction loss tend to produce images which are
blurry, one can train an adversarial autoencoder (Makhzani et al., 2016), but instead of putting the
adversary on the bottleneck, we put it on the reconstruction, and the discriminator (denoted $D_{\omega}(\hat{x}$) tries
to predict the mixing coefficient $\alpha$ that was used to generate the decoded signal. It outputs a scalar value and is trained to minimize
\begin{equation}\label{eq:lossDiscriminator}
    L_d = \underbrace{||d_\omega (\hat{x}_\alpha) - \alpha ||^2}_\text{predict $\alpha$} + \underbrace{||d_\omega (\gamma x + (1 - \gamma)\hat{x}||^2}_\text{stabilizes training}.
\end{equation}
where $\gamma$ is a scalar hyperparameter.



%% Novel Contribution / Limitation
To illustrate the \acronym in the context of clustering, we first discuss an example of linear interpolations between four classes, depicted in figure \ref{fig:interpolation}. When interpolating between two clusters, for example from cluster B to cluster C, the resulting interpolant will likely look like a realistic data point of cluster B and become less semantically similar to B and more semantically similar to C as a function of increasing $\alpha$. Since an interpolant always has to look like a realistic datapoint, interpolants close to cluster B will look like a real data point from B whereas an interpolant close to cluster C will look like a real datapoint from C, visualized as blurred versions of the cluster's datapoints in figure \ref{fig:interpolation}. However, let's consider the outlier of cluster B at the right end of the coordinate system. If we'd like to interpolate this data point with another data point from cluster C, the interpolants with an $\alpha \approx 0.5$ will not necessarily look like a real data point from the clusters B or C, but instead it would look like a data point coming from cluster D. This is because, for $\alpha \approx 0.5$, the position of the interpolated data point would lie in the area where most data points belong to cluster D (bottom right quadrant of the coordinate system in figure \ref{fig:interpolation}) and, therefore, through interpolations of data points from D with other clusters, interpolants in this quadrant will look most similar to D. Since the interpolant will look like a realistic datapoint, the discriminator will output $\alpha = 0$ and the overall loss of the autoencoder would not increase without the added constraint. In other words, any realistic looking interpolant between cluster C and B will correspond to an inability of the critic to guess the used $\alpha$ value. 
However, this behaviour would not explicitly enforce linear dependencies between clusters, which is an important characteristic of disentangled representations \cite{bengio2013representation}. Additionally, this also means that the network would not necessarily need to create more disentangled clusters because the described behaviour would not enforce the creation of low density regions between clusters. In the above scenario, the outlier from cluster B does not have any 'incentive' to move towards the cluster centroid but can stay at its position. Instead, we would like the data point to move towards the centroid position to enforce lower density regions between clusters.

\begin{figure}[h]
\centering
\includegraphics[width=6cm,height=5cm]{Figures/interpolation_WITHOUT_GRAD.png}
\caption[Example Interpolation]{Illustration of linear interpolations and low-density regions between four clusters of classes.} 
\label{fig:interpolation}
\end{figure}

\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.8]{Figures/acai_vs_acai+/two_MNIST_all.png}
    \caption[Example Interpolation]{The models' learned data point positions in the two-class MNIST example.}
    \label{fig:two_mnist_example}
\end{figure*}

To enforce the desideratum of linear dependencies between clusters, we propose \acronym, which introduces an additional constrained that is added to the overall loss function of the autoencoder. More specifically, when linearly interpolating between $x_1$ and $x_2$, the interpolants for $\alpha \in [0, 0.5]$ must look like $x_1$ whereas the interpolants for $\alpha \in [0.5, 1]$ must look like $x_2$. Formally, this can be expressed by:
\begin{equation}
    z_\alpha = (1 - \alpha) f_\phi (x_i) + \alpha f_\phi (x_j)
\end{equation}
\begin{equation} \label{eq:addedConstraint}
    L = || x_i - g_{\theta}(z_{\alpha}) ||^2   
\end{equation}
where $\alpha \in [0, 0.5]$. Consequently, we define the overall loss function of the autoencoder as follows:
\begin{equation}
    L_{i} = || x_i - g_{\theta}(f_{\phi}(x_i)) ||^2 + \lambda ||d_\omega (\hat{x}_\alpha) ||^2 + || x_i - g_{\theta}(z_{\alpha}) ||^2
\end{equation}
This overall loss should enforce that all clusters can linearly interpolate between each other and, in addition, that all interpolants look like coming from the respective data points that were used for the interpolation. Turning to the interpolation between the outlier of cluster B and a data point from C, the resulting interpolant will look like a realistic data point from D, which is not one of the input images and, as a consequence, the autoencoder loss will increase. Since every position in the coordinate system can only store a single representation (i.e. the position of the interpolant in the coordinate system can only be decoded deterministically as a datapoint coming from one of the clusters B, C, or D), there will be a conflict of assigning different representations to the same position. As the datapoint locations are learned through training, it is expected that the pressure to decode consistent representations at interpolated positions causes the outlier from cluster B to move towards the centroid position of cluster B. Eventually, this would lead to more disentangled clusters and lower-density regions between the clusters.












\begin{comment}
distinguish between real and reconstructed $x$, and the autoencoder tries to construct 'realistic' reconstructions so as to fool the discriminator. For this formulation, we coin the term 'AE + GAN'. This can be written as:

\begin{equation}
    \min_{F} \mathbb{E}_{x\sim p(x)} \lambda|| x - g(f(x))||_2 + \ell_{GAN}(D(g(f(g))), 1)
\end{equation}
\begin{equation}
    \min_{D} \mathbb{E}_{x\sim p(x)} \ell_{GAN}(D(x),1) + \ell_{GAN}(D(g(f(x))),0),
\end{equation}
where $\ell_{GAN}$ is a GAN-specific loss function. In our case, $\ell_{GAN}$ is the binary cross-entropy loss, which corresponds to the Jenson-Shannon GAN (QUOTE GOODFELLOW).


What we would like to do is to be able to encode an arbitrary pair of inputs $h_1 = f(x_1)$ and $h_2 = f(x_2)$ into their latent representation, perform some combination between them through a function we denote $Mix(h_1, h_2)$(more on this soon), run the result through the decoder $g(z,\theta)$, and then minimise some loss function which encourages the resulting decoded mix to look realistic. With this in mind, we propose AMR, where part of the aut-encoder's objective is to produce mixes which, when decoded, are indistinguishable from real images. The generator and the discriminator of AMR are trained by the following mixture of loss components:

\[
  \min_{F} \mathbb{E}_{x, x' \sim p(x)} \underbrace{\lambda ||x-g(f(x))||_2}_\text{reconstruction} + \underbrace{\ell_{GAN}(D(g(f(x))),1)}_\text{fool D with reconstruction} + \underbrace{\ell_{GAN}(D(g(Mix(f(x), f(x')))),1)}_\text{fool D with mixes}
\]
\[
  \min_{D} \mathbb{E}_{x, x' \sim p(x)} \underbrace{\ell_{GAN}(D(x),1}_\text{label x as real} + \underbrace{\ell_{GAN}(D(g(f(x))),0)}_\text{label reconstruction as fake} + \underbrace{\ell_{GAN}(D(g(Mix(f(x), f(x')))),0)}_\text{label mixes as fake}
\]

There are many ways one could combine the two latent representations, and we denote this function $Mix(f_{\phi}(x_1), f_{\phi}(x_2)$. Manifold mixup (Verma et al., 2018) implements mixing in the hidden space through convex combinations:
\begin{equation}
    z_{\alpha} = \alpha f_{\phi}(x_1) + (1-\alpha) f_{\phi}(x_2),
\end{equation}
where $\alpha \in [0,1]$ is sampled from a Uniform(0,1) distribution. We can interpret this as interpolating along line segments, as shown in Figure X.


\subsection{ACAI}\label{sec:methods_acai}
Recently, Berthelot and colleagues \citep{berthelot2018understanding} proposed a method to apply interpolation training in an unsupervised setting. In their ACAI framework, interpolating describes the process of using an encoder $f_{\phi} (x)$ to map datapoints onto a lower-dimensional latent representation $z$. A decoder $g_{\theta}(z)$ is then used to reconstruct a mixture of two latent representations. For two datapoints $x_1$ and $x_2$, the linear interpolation $z_{\alpha}$ is calculated as:
\begin{equation}
    z_{\alpha} = \alpha \cdot f_{\phi} (x_1) + (1 - \alpha) \cdot f_{\phi} (x_2)
\end{equation}
for some $\alpha \in [0,1]$. The resulting interpolated representation $z_{\alpha}$ is then reconstructed by the decoder $\hat{x}_{\alpha} = g_{\theta} (z_{\alpha})$. Ideally, adjusting $\alpha$ from 0 to 1 will produce a sequence of realistic datapoints where each subsequent $\hat{x}_\alpha$ is progressively less semantically similar to $x_1$ and more semantically similar to $x_2$. Then, a second encoder network $d_{\omega}$, called a \textit{critic} or \textit{adversarial regularizer}, is fed these interpolants and its goal is to predict the mixing coefficient $\alpha$ that was used to generate the decoded signal. More formally, it outputs a scalar value and is trained to minimize
\begin{equation}\label{eq:lossDiscriminator}
    L_d = ||d_\omega (\hat{x}_\alpha) - \alpha ||^2 + ||d_\omega (\gamma x + (1 - \gamma)\hat{x}||^2
\end{equation}
where $\gamma$ is a scalar hyperparameter. The first part of the equation calculates the MSE between the predicted and true $\alpha$ values whereas the second part of the equation predicts the $\gamma$ hyperparameter that is used to interpolate between the input image $x$ and the reconstruction $\hat{x}$ \footnote{\cite{berthelot2018understanding} suggest that this second term may not be necessary but helps to stabilize the training process in the early training phase.}. Simultaneously, the autoencoder is trained to fool the critic to think that the $\alpha$ value is always zero and it receives the critic's performance as feedback in terms of a loss. Consequently, the overall loss of the autoencoder is
\begin{equation}\label{overallAutoencoderLoss}
    L_{f,g} = || x - g_{\theta}(f_{\phi}(x)) ||^2 + \lambda ||d_\omega (\hat{x}_\alpha) ||^2
\end{equation}
where $\lambda$ is a hyperparameter that determines how strongly the critic's performance contributes to the overall autoencoder loss. Empirically, this approach resulted in realistic and smooth interpolations of the autoencoder's latent space as well as in increased clustering accuracy \cite{berthelot2018understanding}.

\end{comment}
